Arbitrary Pattern Formation on Infinite Regular Tessellation Graphs

Given a set R of robots, each one located at different vertices of an infinite regular tessellation graph, we aim to explore the Arbitrary Pattern Formation (APF) problem. Given a multiset F of grid vertices such that |R|=|F|, APF asks for a distributed algorithm that moves robots so as to reach a configuration similar to F. Similarity means that robots must be disposed as F regardless of translations, rotations, reflections. So far, as possible graph discretizing the Euclidean plane only the standard square grid has been considered in the context of the classical Look-Compute-Move model. However, it is natural to consider also the other regular tessellation graphs, that are triangular and hexagonal grids. We provide a resolution algorithm for APF when the initial configuration is asymmetric and the considered topology is any regular tessellation graph.

==> fig/T1.1 <==
#FIG 3.2  Produced by xfig version 3.2.7a
Landscape
Center
Inches
Letter
100.00
Single
-2
1200 2
0 32 #aaaaaa
0 33 #bbbbbb
0 34 #cccccc
0 35 #999999
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 7794 1500 48 48 7794 1500 7842 1500
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 7530 1057 48 48 7530 1057 7578 1057
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 8055 135 48 48 8055 135 8103 135
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 7538 143 48 48 7538 143 7586 143
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 7794 600 48 48 7794 600 7842 600
1 3 0 2 0 -1 45 -1 20 0.000 1 0.0000 8558 142 30 30 8558 142 8588 142
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 5475 150 48 48 5475 150 5523 150
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 3646 1492 48 48 3646 1492 3694 1492
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 3382 1049 48 48 3382 1049 3430 1049
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 3907 127 48 48 3907 127 3955 127
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 3390 135 48 48 3390 135 3438 135
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 1567 592 48 48 1567 592 1615 592
1 3 0 2 0 34 45 -1 20 0.000 1 0.0000 3646 592 48 48 3646 592 3694 592
1 3 0 2 0 -1 45 -1 20 0.000 1 0.0000 4410 134 30 30 4410 134 4440 134
2 1 1 2 35 7 52 -1 -1 4.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 5196 150 9223 150
2 1 1 2 35 7 52 -1 -1 4.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 7274 2400 8898 -412
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7274 -300 6235 1500
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5455 150 8573 150
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7794 -300 9092 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8573 150 7533 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5715 -300 7014 1950
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8313 -300 9612 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8832 612 8053 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9092 1062 8573 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9352 1512 9093 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6754 -300 5975 1050
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7274 -300 8572 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6495 1950 9611 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6235 -300 5710 610
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6235 1500 9352 1512
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5715 600 8832 612
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5196 -300 8313 -300
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5715 -300 5450 159
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6754 -300 8053 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5196 -300 6500 1959
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8313 -300 7014 1950
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7794 -300 6495 1950
2 3 0 2 4 7 55 -1 -1 0.000 0 0 -1 0 0 5
	 7525 158 7005 1058 7545 1058 8048 157 7525 158
2 3 0 2 4 7 55 -1 -1 0.000 0 0 -1 0 0 5
	 3386 142 2606 1492 3638 1484 4425 142 3386 142
2 3 0 2 1 7 55 -1 -1 0.000 0 0 -1 0 0 5
	 2864 142 3644 1492 4685 1492 3906 142 2864 142
2 1 1 1 35 7 52 -1 -1 4.000 0 0 -1 0 0 2
	 1567 1492 5542 1507
2 1 1 1 35 7 52 -1 -1 4.000 0 0 -1 0 0 2
	 1307 1042 5295 1049
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3126 -308 2087 1492
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1307 142 4425 142
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1827 1042 4944 1054
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3646 -308 4944 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 4425 142 3385 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1567 -308 2866 1942
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 4165 -308 5464 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 4684 604 3905 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 4944 1054 4425 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5204 1504 4945 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2606 -308 1827 1042
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3126 -308 4424 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2347 1942 5463 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2087 -308 3385 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2087 -308 1562 602
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2087 1492 5204 1504
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3646 -308 2347 1942
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1567 592 4684 604
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1048 -308 4165 -308
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1567 -308 1302 151
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2606 -308 3905 1954
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1048 -308 2352 1951
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 4165 -308 2866 1942
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6235 -300 7533 1962
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5975 1050 9092 1062
2 1 1 1 35 7 52 -1 -1 4.000 0 0 -1 0 0 2
	 849 142 4837 142
4 0 35 60 -1 0 12 0.0000 6 180 360 8576 345 $O$\001
4 0 35 60 -1 0 12 0.0000 6 210 585 8963 -75 $Q^+$\001
4 0 35 60 -1 0 12 0.0000 6 180 345 8668 -412 $Y$\001
4 0 35 60 -1 0 12 0.0000 6 180 360 9077 359 $X$\001
4 0 0 60 -1 0 12 0.0000 6 210 495 7879 1702 $r_6$\001
4 0 0 60 -1 0 12 0.0000 6 210 495 5550 375 $r_1$\001
4 0 0 60 -1 0 12 0.0000 6 210 495 1697 517 $r_1$\001
4 0 0 60 -1 0 12 0.0000 6 210 555 1307 1417 $L_2$\001
4 0 0 60 -1 0 12 0.0000 6 210 585 3970 29 $r''_6$\001
4 0 0 60 -1 0 12 0.0000 6 210 600 1048 967 $L'_2$\001
4 0 0 60 -1 0 12 0.0000 6 210 1065 398 67 $L_1=L'_1$\001
4 0 0 60 -1 0 12 0.0000 6 180 375 3956 1207 $S'$\001
4 0 0 60 -1 0 12 0.0000 6 180 420 4346 892 $S''$\001
4 0 0 60 -1 0 12 0.0000 6 210 540 3731 1694 $r'_6$\001
4 0 35 60 -1 0 12 0.0000 6 210 525 6218 2176 $Q^-$\001
4 0 35 60 -1 0 12 0.0000 6 180 540 7125 1014 $P^*$\001

